The Jasper Framework: Towards a Platform Independent, Formal Treatment of Web Programming

This paper introduces Jasper, a web programming framework which allows web applications to be developed in an essentially platform indepedent manner and which is also suited to a formal treatment. It outlines Jasper conceptually and shows how Jasper is implemented on several commonplace platforms. It also introduces the Jasper Music Store, a web application powered by Jasper and implemented on each of these platforms. And it briefly describes a formal treatment and outlines the tools and languages planned that will allow this treatment to be automated.

==> eptcsdata.tex <==
\providecommand{\firstpage}{31}
\providecommand{\publicationstatus}{J. Silva and and F. Tiezzi (Eds.): Workshop on Automated\\ 
Specification and Verification of Web Systems (WWV 2012)\\
EPTCS 98, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.98.5}{10.4204/EPTCS.98.5}}
\pdfoutput=1

